Managing Large-Scale Transient Data in IoT Systems

The pervasive availability of streaming data is driving interest in distributed Fast Data platforms for streaming applications. Such latency-sensitive applications need to respond to dynamism in the input rates and task behavior using scale-in and -out on elastic Cloud resources. Platforms like Apache Storm do not provide robust capabilities for responding to such dynamism and for rapid task migration across VMs. We propose several dataflow checkpoint and migration approaches that allow a running streaming dataflow to migrate, without any loss of in-flight messages or their internal tasks states, while reducing the time to recover and stabilize. We implement and evaluate these migration strategies on Apache Storm using micro and application dataflows for scaling in and out on up to 2-21 Azure VMs. Our results show that we can migrate dataflows of large sizes within 50 sec, in comparison to Storm's default approach that takes over 100 sec. We also find that our approaches stabilize the application much earlier and there is no failure and re-processing of messages.

==> approach.tex <==
\section{SINC Framework}\label{sec:approach}
We approach the above-mentioned issues by designing a framework named
Slicing IoT, Network Functions and Clouds (SINC). The goal of the
framework is to provide fundamental building blocks to enable the creation,
management and adaption end-to-end slices of diverse types of
resources from IoT, network functions and clouds for particular
customers based on their functional and non-functional requirements. 
\begin{figure*}[htbp]
\centering
\includegraphics[width=1.0\linewidth]{conceptual-architecture.pdf}
\caption{Slicing IoT, Network Functions, and Clouds (SINC) -- Conceptual Architecture}
\label{fig:arch}
\end{figure*}
\subsection{Conceptual Architecture}\label{subsec:arch}

The overall conceptual architecture of our framework is as depicted in
Fig.~\ref{fig:arch}. We envisage the existence of a user request
provisioning component at the {\em Application} layer (the top layer
in Fig.~\ref{fig:arch}), which is essentially a placeholder for a
component that processes user requests and invokes the appropriate
components in our SINC framework. Typical applications for our
framework would be emergency application, on-demand sensing, sport
event management, to name just a few. We also envisage the
availability of different types of {\em IoT Networks}, {\em Network
  Function Services} and {\em Clouds} infrastructures, shown at the
bottom of Fig.~\ref{fig:arch}. These types of infrastructures can be
simple or complex, e.g., an IoT network might just consist of a set of
public sensors that can access directly or a set of pay-per-use
sensors, actuators and gateways offered under the service model
\cite{Perera:2014:SSM:2855057.2855066}. Similarly, Network Function
Services might be provided by an on-demand micro data center
\cite{Laoutaris:2008:EEC:1341431.1341442,DBLP:conf/mobicase/EcheverriaRBL14}
connected to telco networks or complex network function virtualization
services offered by telcos in the fog computing model
\cite{bonomi2012fog}.  These infrastructures provide different types
of resources and these resources will be accessible and controllable
through well-defined APIs. 

The SINC framework will include three layers: (i) {\em API Integration
  and Communication}, (ii) {\em Naming, Slicing and Routing}, and
(iii) {\em Resource Management, Configuration, and Adaptation}. We
devise {\em API Integration and Communication} for integrating and
communicating existing infrastructures of sensors, edge-to-cloud and
cloud resources, each from different vendors, whereas {\em Resource
  Management, Configuration and Adaptation} is meant for specific operations on
provisioning end-to-end  slices for the applications. The {\em Naming,
  Slicing and Routing} layer comprises components for
information-centric provisioning partially derived
from~\cite{amadeo2014named}. The Naming component is responsible for
assigning identities to virtual resources, such as virtual sensors or
virtual networks. It also maintains mappings to the actual underlying
physical resources. The Slicing component performs the actual task of
virtualizing the network resources as well as defining and
provisioning the network slice to meet the user needs. During actual
operation, it invokes the Routing component to route data through the
network slice components. The actual routing and transport is
performed by {\em API Integration and Communication} components, which
interface with network layer components such as gateways, routers and
virtual sensors. In the next subsections, we will elaborate these layers and components  and outline our effort towards an implementation of SINC.

%SINC is a conceptual framework, thus we expect to have different routes to its implementation. In the next subsections, we will elaborate these layers and components in detail and outline our effort towards an implementation of SINC. 
%The latter in turn are the only components that directly interface with the actual IoT devices, for both sensing and actuation. Indeed, Fig.~\ref{fig:arch} also depicts an instantiation of end-to-end IoT network slicing for integrated provisioning of sensors, edge-to-cloud and cloud resources, each from different vendors.



\subsection{API Integration and Resource Management}

\subsubsection{API Integration}
The first step in our framework is the capability to integrate different APIs from existing infrastructures so that we can access diverse resource capabilities and manage these capabilities. In this sense, in the {\em API Integration and Communication} layer, {\em API Integration} will include a collection of APIs for accessing and managing resources so that we can negotiate and procure resource capabilities and invoke and monitor them. It is important to note that there are many APIs from different infrastructures (and their providers), however, we do not need to consider all of them. In the SINC framework, only needed APIs will be included. In this view, we could leverage API management services \cite{Vukovic:2015:IPI:2843962.2822873, Cho:2013:IMS:2494621.2494648,Vukovic:2016:RTA:2897191.2816812} within a SINC implementation to support the integration with existing infrastructures.

\subsubsection{Communication Middleware}
Since we will have requests and commands from high-level components to
concrete resources in different, distributed infrastructures, {\em
  Communication Middleware} is needed to support different types of
communication. This middleware works together with API integration to
invoke suitable APIs to transfer (meta)data about resources and commands. However, it has to
deal with different types of interactions. Therefore,  this requires
us to develop a loosely coupled communication middleware based on
matured technologies for inter-cloud and IoT communication, such as
AMQP \cite{amqp}, CoAP \cite{coap}, and MQTT \cite{mqtt}. In SINC, the {\em Communication Middleware} is for managing resources. Therefore, we envisage different  middleware for transferring actual data produced by sensors to cloud services. 

\subsubsection{Resource Grid}
Through {\em API Integration} and {\em Communication Middleware} we
could have an instant view on  available resources from existing
infrastructures. Such available resources might be just a subset of
existing resources in these infrastructures (since the providers might
not make all resources available for the application).  We need {\em Resource Grid} to  provide a map to
underlying resources that are available to applications using the
end-to-end slice approach. {\em Resource Grid} presents resources to
components in the {\em Naming, Slicing and Routing} layer by
harmonizing diverse types of information representations.  Depending
on the implementation, {\em Resource Grid} may just mirror all
available resources through APIs -- so it may just perform the
transformation and harmonization of information through API calls -- or it
may replicate information about resources in SINC by querying, 
pulling and caching information from existing infrastructures. Overall, {\em Resource
  Grid} just keeps a portion of resources that individual providers
make available for end-to-end slicing. 
%
%Information in resource grid allows us to use middleware and apis to tell the underlying providers what we want. On the other hand, allow us to build high-level information-centric resource for naming.

\subsection{Naming, Slicing and Routing}

%%We now discuss a few key components in some detail and discuss how they could be designed.

%\subsection{Naming}\label{subsec:naming}

\subsubsection{Naming} As enunciated in~\cite{amadeo2014named}, the
information-centric approach enables the use of application-specific
names. However, this naming scheme should be broad enough so that it
can be understood by users spanning various application domains. The
naming hierarchy should also be explicitly specified, e.g.,
$/city\_name/bangalore/street\_name$
$/cunningham\_road/location/20/corner/east$
$/sensor\_type/video/sensorID/1$, may refer to video camera sensor \#1
stationed 20 feet from the beginning of Cunningham Road in the city of
Bangalore. Multiple such video camera sensors could be positioned
along Cunningham Road, and would form part of a virtual sensor with
name $/city\_name/bangalore/street\_name/$
$/cunningham\_road/sensor\_type/virtual/sensorID/A$.  

In our approach, we will utilize this naming strategy for all
resources in the IoT system, including IoT devices (sensors \&
actuators), network services \& equipment, and cloud services. Indeed,
if many (cloud) computing and/or storage functions are moved to the edge as
described in~\cite{haubenwaller2015computations}, this naming strategy
would be needed. Using this naming, we can easily describe and
identify the data, computing and network capabilities of diverse types
of resources. However, a challenge is that the composition of these
resources for an end-to-end provisioning would also rely on many other types of 
information, such as geographical distribution, connection
performance, availability, and security and privacy attributes. In this case, naming
for resources gathered from underlying systems will also link to such
(meta and monitoring information) for determining optimal
compositions.    


\subsubsection{End to End Slicing}: As stated earlier, and as depicted
in Fig.~\ref{fig:arch}, network slicing in our case encompasses the
\emph{entire} IoT system. Typical proposed network slicing approaches
as in~\cite{inam2015towards} limit themselves to only the core network
equipment infrastructure, with some integration to backend cloud
infrastructure. Indeed,~\cite{inam2015towards} does present a
prototype implementation on
Openstack \cite{openstack}. However, our approach
would need to provide a higher-level service orchestration mechanism
through the utilization of specific mechanisms for {\em partitions} of
IoT, network
functions, and clouds as well as through the new development of such
combined mechanism. In our approach, slicing techniques for IoT and
cloud partitions would focus on mechanisms to provision guaranteeing data and
computing capabilities (e.g., dedicated sensors, gateways, and virtual
machines). Slicing techniques for network function partitions will focus on
network capabilities between (i) existing nodes of IoT subnetworks
connecting to access nodes of the network functions in the middle and
(ii)existing nodes of the network functions in the middle and the
access node of the cloud data centers.  
As a result of slicing techniques, resources in end-to-end slices can be described,
deployed and configured 
by techniques such as
TOSCA \cite{tosca}, and service
chaining \cite{servicechaining},
the latter for instantiating and interconnecting virtual network
functions to form a service.  

%\subsection{Routing and Transport}\label{subsec:routing}

\subsubsection{Routing} Typical routing infrastructure in ICN
comprises the following
components~\cite{amadeo2014named,amadeo2015information}: (i) a Content
Store (CS) for temporary caching of incoming Data packets; (ii) a
routing table called Forwarding Information Base (FIB) used to guide
the Interests towards Data; and (iii) a Pending Interest Table (PIT),
which keeps track of the forwarded Interest(s) that are not yet
satisfied with a returned data packet. Our goal is to  utilize these concepts
for routing data and requests among resources provisioned for
slices. This means that we need to carefully investigate how to
implement these concepts at the level of (virtualized) resources in
slices. Essentially, as we have different partitions of resources
identified by the {\em Naming} component that can be accessed and controlled
through the {\em Communication Middleware}, all of these concepts will
be implemented atop an overlay network of resources. Hence, routing
can be two-way, i.e., the FIB can also be 
used to route commands to sensors and actuators, for implementing 
actuation commands, e.g., changing the data rate of a sensor, or
changing the unit of a body temperature sensor from Centrigrade to
Fahrenheit. The key issue in the design 
here is that the routing has to be accomplished 
within certain limits (based on QoS considerations), and has to be
accomplished reliably. At the higher-level, this, however, depends on
the capabilities of the {\em Communication Middleware} which carry
requests and data. At the lower level, this depends on the properties of the
selected end-to-end network slice, in particular, its bandwidth
capacity, its topology, and the latency of data transmission within
the slice. Since multiple slices may have to be implemented
simultaneously based on user needs, this becomes a dynamic
optimization problem that needs to be solved within the constraints of
the selected network slice.  


\subsection{Managing End to End Slices}
As we have seen above, the end to end network slice, encompassing
sensors, network functions and cloud resources, would become the most
crucial entity of our IoT network. Hence it needs to be managed
effectively. This involves the following: creation and deployment of
the slice, distributed monitoring and management of the resources that
make up the slice, and adaptation of the slice in response to changing
user requests and/or changing network environment. 

\subsubsection{Creation and Deployment}\label{subsec:creation}
The process of creation of a slice would start with the user
specifying their requirements for the following: data needed from
sensors, minimum network bandwidth needed, backend compute and storage
needed. For example, the user may ask for data from a set of traffic
sensors every 5 minutes, at least network bandwidth of 16 MB per
second, backend compute capacity of at least 16 GB of memory, and
backed storage of at least 1 TB. The user may also request this
functionality for 4 hours, for e.g., for the time it would take to
complete evacuating the victims in our running example, providing them
first aid en route to hospitals, and monitoring their condition in the
hospitals until they are declared stable and out of danger. 

There are also scenarios where such user requests may be placed well
in advance~\cite{inam2015towards}, e.g., a rock concert or football
match, whose organizers may request dedicated network bandwidth so
that attendees can obtain live information feeds on their
smartphones. Hence in a situation such as our emergency response
scenario, if network bandwidth or compute capability happens to be
insufficient, then lower priority user requests (rock concert) may
have to be de-provisioned in favor of a higher priority request
(emergency response). 

Fulfilling such a request would require the development of a dedicated
service that can integrate with NFV orchestrators, virtual
sensors, gateways, cloud APIs and SDN controllers. Such a service also
has to deal with different resource provisioning models imposed by
underlying infrastructures. For example, it is possible that
underlying infrastructures offers pay-per-use resources with or
without negotiation as well as opportunistic resources through
spot sensors and machine instances. Similarly, deployment for slices
would need to address different deployment models for IoT and clouds,
which are quite different.  

\subsubsection{Distributed Resource Monitoring and Management}\label{subsec:resourcemanagement}

%we will outline some issues about resource management - things that we learn from HINC.

Once the slices have been created, the next step is to monitor the
resources that make up the slice and ensuring that they are performing
as intended. There are two ways in which this monitoring can be
implemented - pull and push. In the former approach, the monitoring
application at the resource management layer of Fig.~\ref{fig:arch}
directly polls the  resources -- sensors, network elements, cloud
resources -- via the API integration layer. The polling frequencies, as
well as extent of status data to be sent by the IoT resources, are
detailed design choices that need to be made depending on the slice in
question. 

Naturally, we foresee the need to integrate different monitoring
systems for IoT, network functions and clouds
\cite{DBLP:conf/bigdataconf/TrihinasPD15,Aceto:2013:SCM:2489309.2489421,DBLP:journals/ijbdi/MoldovanCTD15}. From
the monitoring data, using information from naming, we will correlate
monitoring information from different sources to provide an end-to-end
view on performance of slices. In addition to solving the complexity
of monitoring metric spaces (IoT, network, cloud metrics), we also
have to deal with the complexity of measurement granularity of metrics.  

\subsubsection{Runtime Slice Adaptation}

%how we deal with the monitoring and adaptation of the slice

As is the case with any complex software-defined system, issues will
constantly arise during execution, that demand runtime adaptation. In
our case, we can identify two key issues: changes in user
requirements, and changes in the underlying infrastructures. These
can be handled in either of two ways: either the change can be
regarded as a new requirement, for which a fresh slice is provisioned
(as described above); or the slice can be reconfigured at runtime. In
particular, changes in the underlying  infrastructures -- such as
unavailability of network equipment, breakdown in underlying network
or sensor hardware, etc. -- would require runtime slice reconfiguration
to ensure continuity. 

A running slice has many points, existing in different slice partitions,  at which reconfiguration can be
implemented, such as: provisioning additional compute and/or storage
at the cloud backend; provisioning additional network bandwidth;
rerouting network traffic using SDN controllers to ensure adherence to
customer needs in the presence of network equipment failure,
redefining virtual sensor data in the presence of failure of
sensors. The last example is particularly interesting; consider, for
example, a set of load sensors on a bridge providing load data. If a
subset of them fail, the virtual sensor that collates this data needs
to perform suitable data interpolation in order to compensate for the
lost sensor data. 

Besides performance, reliability and availability adaptation for
slices, an important aspect of monitoring and management of slices is
to deal with uncertainties \cite{DBLP:conf/icst/AliY15} which are not
well studied in an integrated virtualized IoT, network functions and
cloud-based environment. On the one hand, adaptation techniques have
to deal with monitoring data and actuation uncertainties
\cite{DBLP:conf/cloudcom/NasticCTD15}. On the other hand, they must
deal with the uncertainties in resource behavior. To deal with this
problem, further uncertainties inherent in slices must be studied.  
%\subsection{Providing view of provisionin resources}

%here we need (i) leverage existing APIs from existing IaaS, including clouds, iot, network to build a view. first how to utilize existing APIs
%\subsubsection{Integrating IoT, NFV Orchestration and Routing, Cloud APIs}\label{subsec:nfv}

%\subsubsection{Naming}\label{subsec:naming}
%how naming is used to provide a uniform view

%\subsubsection{APIs for common views}

%we propose to have a common view/API for information-centric resources (by utilizing naming and existing APIs described above.

%\subsection{HINC-End-to-End Slicing Framework}

%here we talk about components in the framework, e.g., composition, slicing, etc.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\linh{do we follow the conceptual approach? If yes, we can draw a conceptual architecture}

%\subsection{Approach}

%To be able to provision an end-to-end slice (\linh{working term - we should fix it later}, the providers should provide several features to allow us to utilize these features to create an end-to-end slides:

%\begin{itemize}
%\item information-centric resource capabilities:  (related to challenge xyz). This relates to (i) resource information model and (ii) APIs. IoT providers have problems as both of them are not well-developed (mostly we access these resources from cloud middleware or low-level protocols, also resources are too low-level). Network providers: APIs are currently available but not widely exposed ? Cloud are clear.
%\item resource provisioning algorithms: \linh{we focus on the discussion of two approaches}. two approaches: one is to leverage existing aglorithms for individual types of infrastructures (iot, cloud, nfv). Which algorithms are available that can be used? How to combine them? Another approach is to consider a ``flat'' view of resources from different systems: we merge and unite all resources from iot, network, and cloud to have a superset of resources. Then we develop the algorithms atop of them. Very challenges! No existing at the moment. 
%Furthermore, end-to-end slices can be optimized. how? we do not know yet (and maybe do not discuss a lot)

%\item create topologies and configure resources to have an end-to-end slice: from the algorithms how do we interact with existing infrastructures to create an end-to-end slice --> we need to invoke complex APIs. 

%\item maintain the slice: the next question is we need to maintain the slice based on quality and cost. how. we can discuss what needs to be done.
%\end{itemize}

\subsection{Towards an Implementation}
%\linh{we try to outline three points: only the first point we have done a bit in HINC}
We envisage different approaches to the implementation of the SINC
conceptual framework due to the complexity and diversity of the underlying IoT, network function services and clouds\footnote{Up-to-date information about SINC implementation is available at \url{http://sincconcept.github.io}.}. We are currently looking into three key aspects for our concrete
implementation. The first aspect is to integrate the diverse IoT
infrastructures and providers at sensor, network function and cloud
levels. We currently make the assumption that all providers would
expose common interfaces and protocols via well-understood
technologies, such as REST API for service interfaces, MQTT and AMQP
for communication, and dockers and OpenStack for virtualization, and
TOSCA/HOT for deployment and configuration. To that end, we are
currently working on a high-level distributed IoT resource information
model and communication middleware, with initial emphasis on IoT
resource monitoring and management~\cite{hinc2016}. 

For naming and routing we are, at an early stage, investigating
integration of techniques from~\cite{amadeo2014named}; in particular,
we will be leveraging the concept of application-specific naming
schemes in the Naming component, and name-based routing in the Routing
component. 

%Naming/Routing/Slicing: we focus on different composition algorithms at IoT \cite{}, networks \cite{} and clouds and at the first step, we are trying to compose them for solving a slice.

For creation and management, we are investigating
TOSCA \cite{tosca} for
describing resources in a slice and existing deployment and
configuration tools slice
deployment\cite{dsg:SALSA-CloudCom,Michael-provisioning}. We will also
be leveraging our ongoing work~\cite{hinc2016} and extending our
monitoring work \cite{DBLP:journals/ijbdi/MoldovanCTD15} for slice
monitoring, and we will be enhancing it for slice adaptation. We are
also investigating Calvin~\cite{NCN:Calvin} as a modeling language for
representing slices as compositions of atomic services. 


%Current monitoring in the cloud, such as \cite{}, are investigated for monitoring slices.  Then programming (Calvin) or using Calvin as a language to describe actions to be executed for controlling the slice


==> challenges.tex <==
\section{Research Challenges}\label{sec:challenges}

%\ncn{Discuss challenges in ICN over IOT, viz., Naming, Distributed Caching, Decoupling between Sender \& Receiver~\cite{lindgren2015applicability}. This should lead to our hybrid ICN+HCN approach in Section~\ref{sec:approach}. Proposed design choices from~\cite{lindgren2015applicability} for IOT over ICN: should work in concert with existing IP protocols; data naming only for directly addressable objects (however, ``virtual'' sensor treatment somehow not very clear - we need to address this in our paper); immutable data objects (of course, our layered ICN+HCN idea should address this issue); how to incorporate data naming for streaming data; should allow for any number of intermediate processing nodes (this should lead us to our layered ICN+HCN idea, and this layering should also ideally be dynamic in nature); capability advertisements (can identify actual *physical* source of data via this, but keep it at lower level of the layered ICN+HCN architecture, and can be virtualized for upper la yers and for end user).}

Many application scenarios require techniques to provision resources
spanning IoT sites, networks and clouds. In these scenarios, users
want to have an end-to-end view of resources so that they can
configure and control resources to make sure that resources fulfill
the requirements given specific contexts, such as, high performance,
high availability, and high throughput. However, considering the
diversity and complexity of resources, users do not want to deal with
host-centric information (e.g., low-level sensor identifier and
network routers).  

Dynamic provisioning of IoT devices (sensors and actuators),
edge-to-cloud network resources, and cloud data center resources as
envisioned in our paper needs to address the following research
challenges before it becomes a reality: 
\begin{itemize}
\item {\em Modeling Distributed IoT, Network Functions and Cloud
  Resource Capabilities}:  resources are of varied types, such as
  sensors, actuators, network elements (routers, gateways, and switches),
  backend cloud resources (compute and storage). In the traditional
  host-centric networking paradigm, each of these resources is
  identified individually and modeled in an information
  model. However, information-centric provisioning requires capability
  modeling at higher abstraction levels. Referring to our running
  example, emergency crews may want to determine the vehicular traffic
  flow through a particular highway, for the purpose of determining if
  there are any blockages. This would require integrated information
  from multiple traffic sensors (road sensors, camera sensors, etc.)
  along the highway, which needs to be presented to the user in
  summarized form. 
\item {\em End-to-End Networks Slicing}: Network slicing is already
  present in implementations such as
  OpenFlow~\cite{salvadori2011generalizing}. However, the end-to-end
  slicing of \emph{all} resources across the edge, the middle and the
  back-end required by implementations such as our running example is
  still an open problem. This would require special techniques for:
  modeling the slice, representing it in memory, reserving resources
  at various levels from different infrastructure-as-a-service in
  order to provision the slice (e.g., sensors, network bandwidth,
  virtual machines, storage), and automatically updating/releasing
  them in response to users' (constantly changing) needs. 
\item {\em Resource Composition in Network Slices}: After end-to-end
  network slicing is implemented, IoT resources have to
  be ``composed'', i.e., provisioned together in a particular sequence
  as per the user's needs. For example, accessing data from a set of
  sensors would require the following resources to be provisioned,
  perhaps in order: network access to intermediate gateway, gateway
  access to ``virtual'' sensor (that collates data from multiple
  sensors), ``virtual'' sensor access to appropriate set of
  sensors. All the while, this will have to be executed over
  virtualized network infrastructure such as OpenFlow, which would
  require implementing multiple path forwarding actions across the
  network slice. 
\item {\em Re-configuring Composed Resources}: After the above
  resource composition is completed, issues could still
  arise. Referring to our running example, a network outage could
  occur in the network slice, perhaps due to a hardware fault in some
  network equipment. This would require dynamically reconfiguring and
  recomposing the network slice by appropriately rerouting network
  flows away from the faulty equipment.  
\end{itemize}

Addressing these issues will create basic building blocks for us to
provision an end-to-end slice of IoT, network functions and cloud
resources. 

\begin{comment}

To enable the provisioning and coordination of resources we need to address:





{\em Resource Identity and Capabilities}: W.r.t IoT, the most important thing is about the information/data capabilities (not low-level resource identity), cloud and network is the same.

so challenges are: mapping from low-level to high-level capabilities

{\em End-to-end Slicing}: how to determine an end-to-end slice and based on which criteria. here we note:
\begin{itemize}
\item based on functional requirements: from in an information-centric approach how do we evaluate existing capabilities to provide an end-to-end
\item based on non-functional requirements: it is very challenging to address costs, security, performance, privacy,
\end{itemize}
 
using composition techniques to compose different resources. This requires (1) composition algorithms, (ii) modeling flows of data and processing actors (through IoT, network, clouds)

{\em Configuration:} we need to access to resource information and APIs to control and configure these resources and to maintain them. (e.g., what if an IoT resource disappears? we need to replace it). It is even more challenges if we reconfigure the end-to-end based on cost and performance. 

\end{comment}


==> intro.tex <==
\section{Introduction}\label{sec:intro}

Driven by advances in sensor networking and mobile computing technologies, Internet of Things (IoT) systems are now becoming prevalent in practically every real-world application domain. Some estimates put the number of IoT devices in the world to about 25 billion by the year 2020 \cite{gartner2014}. %%footnote{\url{http://www.gartner.com/newsroom/id/2905717}}.
Typically, state-of-the-art IoT systems \cite{Botta:2016:ICC:2869179.2869386} comprise three major building blocks: IoT including sensors, actuators, and gateways at the edge, networking equipment and services in the middle, and backend cloud data centers. Such building blocks are also fundamental in mobile-edge-computing, fog computing and cloudlets computing models \cite{Satyanarayanan:2009:CVC:1638591.1638731,Rahimi:2014:MCC:2843689.2843715,etsimec}. These need to be integrated in order to provide usable functionality to users, and are typically provisioned and configured within networks that possess high speed communication capabilities. Moreover, such networks would be large in size, comprising thousands of IoT devices (along with other IoT resources such as gateways, routers, or switches), which, through the networks, communicate with cloud services in data centers.
\subsection{Motivation}
Consider, for example, an emergency response scenario, such as a fire in a crowded theater resulting in several casualties. Such a scenario would require the following:
\begin{itemize}
\item Emergency response services would need to be composed on the
  fly, involving a combination of the following (but not limited to):
  provisioning ambulances, provisioning fire engines, alerting
  doctors, alerting hospitals, and identifying optimal roads/routes to be assigned for emergency vehicles.
\item Victims would be identified and their conditions monitored either by wearable sensors that they are wearing, or wearable sensors that the emergency responders would attach to their bodies.
\item The information from the victims, along with information sent by emergency responders, would inform the appropriate treatment protocols to be administered to the victims on the fly during their transit to the hospital. 
\item Additionally, traffic sensors could point to the most optimal route that emergency vehicles can take, depending on extent of traffic -- although emergency vehicles always have right of way, heavy traffic on certain roads would become difficult to clear quickly enough, especially if there are traffic jams.
\end{itemize}
In such a scenario, we see the need to establish an on-demand IoT
cloud system consisting of several IoT elements at the edge, network
function capabilities in the middle, and cloud services at the
backend. The user of such an IoT cloud system -- the stakeholder who
needs to perform responses to the scenario -- actually wants to have
an end-to-end provisioning of resources spanning from the edge, the
middle, to the back-end, with guaranteed quality of services, due
to the short but crucial workload. With current technologies, such an implementation would require the user to provision each resource -- IoT, network functions, cloud -- separately, and then manually stitch them together, which is a time consuming and error-prone activity.

Similar requirements are also seen in different applications in
cloudlets and mobile-edge-computing models
\cite{DBLP:journals/pervasive/SatyanarayananLMSBH13,etsimec}, such as
on-demand crowd sensing in smart cities \cite{crowdsensing} and performance monitoring in sports
events \cite{utestsportusecase}, when short, high-demand networks and
computing resources are needed. Such a dynamic (and rapid)
provisioning of resources for the IoT cloud system is currently not
possible in current systems, since users would need to rent 
the various components such as sensors, network equipment and cloud
storage separately, and get them integrated via third parties. This is
because most IoT system modeling nowadays is
host-centric~\cite{lindgren2015applicability}, i.e., tied to the
actual host (i.e, source) where particular functionality is
available. Furthermore, virtualization and dynamic provisioning
techniques are investigated for IoT, network functions and cloud
infastructures individually, but not collectively. Thus, creating and
managing end-to-end slices of resources spanning different types of
systems is difficult, if not impossible, with current technologies. 

\subsection{Contributions}

To address the above-mentioned issues, in this paper, we present an
\emph{information-centric}
approach~\cite{amadeo2015information,fotiou2014realizing,DBLP:conf/acmicn/BaccelliMHSW14}
towards IoT (sensors and actuators), network functions and cloud
resource provisioning, which we call \emph{information-centric
  slicing and provisioning}. Such an approach would enable users to, for example,
provision a combination of the following for emergency response crews:
dedicated access to data from specified sensors/wearables, dedicated
network bandwidth, and reserved compute and storage space in cloud
data centers, for as long as they need to complete providing emergency
medical assistance to the fire victims. End-to-end resource slicing
will need to utilize different techniques for different
infrastructures. Thus, for network functions connecting IoT and
clouds, our approach will use 5G network slicing \cite{5gtakingstock,inam2015towards}
to ensure that an end-to-end dedicated ``slice'' of the overall IoT
system (encompassing sensors \& actuators, network infrastructure, as
well as cloud resources such as compute \& storage) is available for
specific requirements (e.g., the emergency response crews), and which
will not face interference from other other existing networking
services offered to the users. Indeed, the approach in~\cite{inam2015towards} shows how network slices can be created by enabling the declarative specification of customer's network requirements, which are then translated into actual physical resource allocation at level of networking equipment.

For IoT and cloud resources, our
approach will use virtualization and on-demand resources provisioning
techniques. Ultimately, we do approach end-to-end resource slicing by
information-centric resource naming, slicing and routing through the
overlay network abstracting and integrating host-centric resource
infrastructures.  

In this paper, we elaborate our approach by contributing  the SINC
framework (Slicing IoT, Network functions, and Clouds) and discuss
main building blocks for SINC  to support the users to create
and manage their end-to-end slices of resources. 
 
\subsection{Paper Structure}
The rest of our paper is organized as follows. In
Section~\ref{sec:challenges}, we discuss some of the research
challenges for provisioning end-to-end slices of resources in IoT systems. In
Section~\ref{sec:approach} we discuss our information-centric approach
for IoT system provisioning and also present our proposed SINC
framework for the same. Section~\ref{sec:relatedwork} positions our
approach against related work in this area, and the paper concludes in
Section~\ref{sec:conclusions} with suggestions for future work. 

%We have observed advanced technologies in three different domains: IoT, network function virtualization and clouds. Currently, there are many novel techniques that enable the integration among them. Examples are ....

%In real-world application domains, such as smart cities, etc.. in order to support these applications, we need techniques that to enable the coordination and provisioning resources among different providers/infrastructures of IoT, network, and clouds. Although, it is possible that one stakeholder can buy and rent these resources from different providers - thus the resources from these providers will be controlled by the stakeholder - currently there is a lack of techniques to support this. While the underlying mechanisms - virtualization, composition, etc - can enable us/the stakeholder to do this, we need to investiage techniques do support them.

%In this paper, we advocate
%\begin{itemize}
%\item a stakeholder or use wants to provision and coordinate resources across IoT, network, and clouds (in the previous work - we discuss a bit the coordination of resources in IoT and clouds, not network)
%\item the stakeholder needs techniques to provision an end-to-end IoT-network-cloud slice by interfacing to underlying infrastructures and providers
%\end{itemize}
%\linh{Why?: we can give a lot of examples}

%In doing so, we believe that composition and coordination techniques could be very useful. 

%Our contributions are:



==> relatedwork.tex <==
\section{Related Work}\label{sec:relatedwork}

\noindent\emph{Information-Centric Networking for IoT}: The concept of virtualizing network topologies in order to enhance efficiency of network utilization has been researched extensively via initiatives such as OpenFlow and OpenDayLight. In particular, in~\cite{salvadori2011generalizing}, the authors presented an innovative system called ``ADVisor''. This system, which extends an earlier network virtualization approach. In particular, it provides the following features: (i) the virtual topologies created are not restricted to specific subsets of the physical topology, and (ii) enables any two slices to share the same flowspace while preserving isolation between them. Works such as~\cite{salvadori2011generalizing} have paved the way for taking a relook at the overall network from an information-centric viewpoint, as presnted earlier in our paper. These are collectively known as Information-Centric Networking or ICN.

Many ICN applications to IoT have been presented. For example, the citation~\cite{fotiou2014realizing} presents a vision for a global, all-encompassing IoT realized through an integrating architecture relying on information and its identifiers/names. They also argue that ICN is the ideal candidate architecture for realizing IoT. They also present several research challenges that need to be overcome before this vision can be realized, viz., naming, efficient and contextual information retrieval, trust modeling, privacy and access control, and information forwarding. A more detailed reification of ICN architectures for IoT is presented in~\cite{amadeo2014named}, which presents a 3-tier architecture comprising application, management+data and thing layers. We have leveraged a few ideas from~\cite{amadeo2014named} in our paper. 

A case study implementation of ICN for IoT in a smart home scenario has been presented in~\cite{amadeo2015information}. In that paper, the authors present a realization of their architecture from~\cite{amadeo2014named}, with emphasis on naming scheme, service model, and strategies for multi-party communications. They also present a preliminary evaluation to provide a rough estimate of ICN based packet communications.

An excellent exposition of ICN and its applicability to IoT is presented in~\cite{lindgren2015applicability}. Apart from discussing the well-known research challenges of ICN, viz., naming, distributed caching and decoupling senders and receivers of data, that paper also discussing specific design choices to be made when ICN is to be used to build IoT systems. A few key choices are: coexistence with existing Internet protocols, using ICN network only for directly addressable data, mandating that IoT uses only immutable data objects, naming data streams so that they can be traced and integrated (e.g., video streams), and representing time-related data streams. We will be considering the design recommendations from~\cite{lindgren2015applicability} for our future papers in this area.

\noindent\emph{Network Slicing and Network-Aware Service Composition}: The other side of the coin in managing IoT systems is network slicing. In our earlier work, we had proposed several principles for engineering cloud-based IoT systems, prominent among them being recommendations for virtualization and composition of IoT components as self-contained units. In this paper, we have incorporated these principles into our proposed conceptual architecture in Fig.~\ref{fig:arch}. These ideas have been leveraged from existing work in network slicing; one such example is described in~\cite{inam2015towards}, which shows how network slices can be created and used. Other works have described in more detail how slices can be created and provisioned~\cite{gutz2012splendid,yiakoumis2011slicing}. A more recent exposition of how network slicing can be implemented in 5G networks is detailed in~\cite{nikaein2015network}.

Recent work has also focused on network-aware service composition~\cite{huang2014qos}, which presents an integrated QoS-aware composition method that integrates application services and network services together. A similar algorithm was also presented earlier in~\cite{Klein:2012}. Extending to the IoT area, recent work has focused on applying network service composition to IoT services. In particular, the citation~\cite{shehu2015network} presents algorithms for IoT service composition that consider not only quality of service (QoS) but also network latency at the IoT application layer. We will be considering these algorithms for implementing our conceptual architecture presented in Fig.~\ref{fig:arch}.

%{\em Virtical IoT models and applications}: \linh{NCN can we discuss about the support of vertical IoT applications - we should have an discussion of end-to-end view}
{\em End-to-end Resource Provisioning}: 
In \cite{Linh:Principles-for-Engineering-IoT-Cloud-Systems}, an end-to-end view on controlling, management and provisioning of IoT and cloud resources is discussed. However, it does not cover h network functions, although it does outline concepts and techniques for creating end-to-end slices of resources. The work in \cite{6654561} discusses the need to have end-to-end network service provisioning across different metro and core network domains. However, it does not focus on end-to-end IoT, network functions and clouds.

%Related work on end-to-end slice: we see individual work in IoT, network and cloud but not and end-to-end (Truong et al. \cite{Linh:Principles-for-Engineering-IoT-Cloud-Systems} discuss an end-to-end view of IoT and clouds but do not include networks which are an important part. 

%Provisioning algoritmhs: any provisioning algorithms for end-to-end slices. The role of composition techniques? networ slicing algorithms \cite{} only focus on networks and currently how to invoke them for end-to-end slices is still not clear. 

%Configuration of end-to-end?

